Mixed Dynamics In Linear Networks: Unifying the Lazy and Active Regimes

The training dynamics of linear networks are well studied in two distinct setups: the lazy regime and balanced/active regime, depending on the initialization and width of the network. We provide a surprisingly simple unifying formula for the evolution of the learned matrix that contains as special cases both lazy and balanced regimes but also a mixed regime in between the two. In the mixed regime, a part of the network is lazy while the other is balanced. More precisely the network is lazy along singular values that are below a certain threshold and balanced along those that are above the same threshold. At initialization, all singular values are lazy, allowing for the network to align itself with the task, so that later in time, when some of the singular value cross the threshold and become active they will converge rapidly (convergence in the balanced regime is notoriously difficult in the absence of alignment). The mixed regime is the `best of both worlds': it converges from any random initialization (in contrast to balanced dynamics which require special initialization), and has a low rank bias (absent in the lazy dynamics). This allows us to prove an almost complete phase diagram of training behavior as a function of the variance at initialization and the width, for a MSE training task.

==> mypreamble.tex <==
\usepackage[utf8]{inputenc}

% Formatting of the page
\usepackage[margin=0.8in]{geometry}
\setlength\parindent{0pt}

% Math Symbols
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{commath}
\usepackage{amssymb}
\usepackage{textcomp}
\usepackage{gensymb}
\usepackage{mathtools}
\usepackage{xcolor}
\usepackage{tikz}\usetikzlibrary{decorations.markings}
\usepackage{tikz-cd}
\usepackage{graphicx,amscd}
\usepackage{mathrsfs}
\usepackage{enumerate}
\usepackage{mathrsfs}
\usepackage{dsfont}
\usepackage{stmaryrd}
\usepackage{wrapfig}
\usepackage{pstricks}
\usepackage{subcaption}
\usepackage{float}

% Code style
\usepackage{listings}
\usepackage{color}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}

% Citations and webpages
\usepackage{natbib}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}

% Miscellaneous
\usepackage{comment}


% New environment wrappers
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{assumptions}[theorem]{Assumptions}

\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{defthm}[theorem]{Definition and Theorem}
\newtheorem*{definition*}{Definition}
\newtheorem*{counterex*}{Counterexample}
\newtheorem*{example*}{Example}
\newtheorem*{exercise}{Exercise}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{observation}{Observation}
\newtheorem*{remark}{Remark}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{example}{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{answer}[theorem]{Answer}

% Shortcuts
\newcommand{\N}{\mathbb{N}} %the set of real numbers
\newcommand{\Z}{\mathbb{Z}} %the set of integers
\newcommand{\Q}{\mathbb{Q}} %the set of rational numbers 
\newcommand{\R}{\mathbb{R}} %the set of real numbers
\newcommand{\C}{\mathbb{C}} %the set of complex numbers
\newcommand{\F}{\mathbb{F}} %notation for field
\newcommand{\A}{\mathbb{A}} %affine space
\renewcommand{\H}{\mathbb{H}} %upper-half complex plane. 
\renewcommand{\P}{{\mathbb{P}}}

\renewcommand{\S}{{\mathbb{S}}} %state space of stochastic process. (p for probability)
\newcommand{\pL}{\mathcal{L}} %probability generator (p for probability)
\newcommand{\cF}{\mathcal{F}} %Filtration (m for measure theory)
%\renewcommand{\E}{{\mathbb{E}}} %Expectation
\newcommand{\cH}{\mathcal{H}}
\DeclareMathOperator{\cov}{Cov}

\newcommand{\sB}{\mathscr{B}} %Borel algebra (m for measure theory)
\newcommand{\f}[1]{\mathfrak{#1}} %maximal ideals
\newcommand{\abra}[1]{\langle #1 \rangle} %inner products and triangle bracket processes. 
\usepackage[shortlabels]{enumitem} %use letters to enumerate items. 
\newcommand{\tor}{\text{Tor}} %Tor functor
\newcommand{\ext}{\text{Ext}} %Ext functor
\newcommand{\into}{\hookrightarrow}
\newcommand{\onto}{\twoheadrightarrow}


\newcommand{\1}{\mathds{1}}
\newcommand{\I}{1\!\!1}                   %Indicator function
\newcommand{\bra}[1]{\left( #1 \right)}
\newcommand{\sbra}[1]{\left [ #1 \right]}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\renewcommand{\max}{\text{max}}
\renewcommand{\min}{\text{min}}
